WxBS: Wide Baseline Stereo Generalizations

We have presented a new problem -- the wide multiple baseline stereo (WxBS) -- which considers matching of images that simultaneously differ in more than one image acquisition factor such as viewpoint, illumination, sensor type or where object appearance changes significantly, e.g. over time. A new dataset with the ground truth for evaluation of matching algorithms has been introduced and will be made public. We have extensively tested a large set of popular and recent detectors and descriptors and show than the combination of RootSIFT and HalfRootSIFT as descriptors with MSER and Hessian-Affine detectors works best for many different nuisance factors. We show that simple adaptive thresholding improves Hessian-Affine, DoG, MSER (and possibly other) detectors and allows to use them on infrared and low contrast images. A novel matching algorithm for addressing the WxBS problem has been introduced. We have shown experimentally that the WxBS-M matcher dominantes the state-of-the-art methods both on both the new and existing datasets.

==> intro.tex <==
%See bmvc_review,tex

==> tables/mtlb_wxbs_solved.tex <==
ASIFT	&-	&0	&52.6	&-	&0	&35.2	&-		&0	&12.1	&-	&0	&30		&-	&0	&32.6	\\
MODS	&1	&-	&\textbf{7.9}	&0	&-	&\textbf{6.52}	&0		&-	&\textbf{2.04}	&1	&-	&\textbf{3.12}	&1	&-	&\textbf{5.75}	\\
DBstrap	&0	&-	&11.7	&0	&-	&13.2	&0		&-	&4.75	&0	&-	&15.5	&0	&-	&13.5	\\
Proposed	&\textbf{4}	&\textbf{3}	&32.7	&4	&3	&36.5	&0		&\textbf{1}	&18.1	&\textbf{2}	&\textbf{2}	&24		&\textbf{3}	&\textbf{2}	&38.2	\\
%WxBS-M2	&3	&1	&16.2	&4	&3	&18.9	&0		&0	&9.41	&\textbf{2}	&\textbf{2}	&14.4	&\textbf{3}	&0	&20.9	\\
%WxBS-M3	&3	&2	&20.7	&2	&\textbf{4}	&23.8	&\textbf{1}		&\textbf{1}	&10		&\textbf{2}	&\textbf{2}	&15.1	&2	&1	&26.4	\\
%WxBS-M4	&3	&\textbf{3}	&32.7	&3	&\textbf{4}	&40.8	&\textbf{1}		&\textbf{1}	&18.3	&\textbf{2}	&\textbf{2}	&26.6	&2	&0	&46.8	\\
%WxBS-M5	&2	&2	&15.6	&3	&\textbf{4}	&20.	5&0		&0	&7.63	&\textbf{2}	&\textbf{2}	&11.1	&\textbf{3}	&0	&17	\\

==> tables/table3.tex <==
\centering{Alg.}& \multicolumn{2}{c|}{EF}
& \multicolumn{2}{c|}{EVD}
& \multicolumn{2}{c|}{MMS}
& \multicolumn{2}{c|}{\textsc{WgABS}}
& \multicolumn{2}{c|}{\textsc{WgalBS}}
& \multicolumn{2}{c|}{\textsc{WglBS}}
& \multicolumn{2}{c|}{\textsc{WgsBS}}
& \multicolumn{2}{c|}{\textsc{WlaBS}}
& \multicolumn{2}{c|}{Past}
& \multicolumn{2}{c|}{OxAff}
& \multicolumn{2}{c|}{SymB}
& \multicolumn{2}{c|}{GDB}
\\
 & \shortstack{\# \\33}& \shortstack{time \\ $[s]$}
& \shortstack{\# \\ 15}& \shortstack{time \\ $[s]$}
& \shortstack{\# \\100}& \shortstack{time \\ $[s]$}
& \shortstack{\# \\ 5}& \shortstack{time \\ $[s]$}
& \shortstack{\# \\8}& \shortstack{time \\ $[s]$}
& \shortstack{\# \\ 9}& \shortstack{time \\ $[s]$}
& \shortstack{\# \\ 5}& \shortstack{time \\ $[s]$}
& \shortstack{\#\\ 4}& \shortstack{time \\ $[s]$}
& \shortstack{\#\\172}& \shortstack{time \\ $[s]$}
& \shortstack{\#\\40}& \shortstack{time \\ $[s]$}
& \shortstack{\#\\46}& \shortstack{time \\ $[s]$}
& \shortstack{\# \\22}& \shortstack{time \\ $[s]$}
\\
\hline
\multicolumn{25}{|c|}{Thresholding strategy}\\
\hline

MSER & 16 & 1.4 & 3 & 1.4 & 1 & 0.3 & 0 & 2.0 & 0 & 1.3 & 0 & 1.3 & 0 & 0.8 & \textbf{1} & 1.2 & 8 & 1.3 & \textbf{40} & 3.5 & 23 & 2.4 & 9 & 2.4\\
AdMSER & 25 & 3.4 & \textbf{8} & 4.0 & 6 & 1.0 & 0 & 4.0 & 0 & 3.2 & 0 & 3.3 & 0 & 1.4 & 1 & 2.6 & 11 & 2.9 & \textbf{40} & 5.7 & 26 & 4.6 & 13 & 6.9\\
DoG & 29 & 2.3 & 0 & 2.8 & 10 & 0.8 & 0 & 2.7 & 0 & 2.3 & 0 & 2.1 & 0 & 1.0 & \textbf{1} & 2.4 & 13 & 2.0 & 38 & 4.8 & 29 & 2.7 & 12 & 4.7\\
iiDoG & 29 & 3.1 & 0 & 3.0 & 11 & 1.2 & 0 & 3.2 & 0 & 2.9 & 0 & 2.8 & 0 & 1.2 & \textbf{1} & 2.5 & 13 & 2.2 & 38 & 8.0 & 29 & 2.9 & 12 & 6.1\\
AdDoG & 29 & 2.6 & 0 & 3.4 & 11 & 1.2 & 0 & 3.3 & 0 & 3.0 & 0 & 3.0 & 0 & 1.5 & \textbf{1} & 2.7 & 13 & 2.7 & 38 & 4.1 & 30 & 3.0 & 12 & 4.8\\
Hes & \textbf{33} & 3.6 & 1 & 6.3 & 26 & 1.6 & \textbf{2} & 5.9 & \textbf{1} & 4.2 & 0 & 4.4 & 0 & 2.2 & \textbf{1} & 3.5 & 35 & 4.5 & 39 & 8.6 & 37 & 6.8 & 18 & 9.9\\
AdHes & \textbf{33} & 5.4 & 1 & 10. & \textbf{60} & 2.7 & \textbf{2} & 10. & \textbf{1} & 8.1 & 0 & 6.6 & 0 & 3.3 & \textbf{1} & 5.3 & \textbf{44} & 5.9  & 39 & 12. & \textbf{39} & 8.7 & \textbf{19} & 14.\\
HesAf & 32 & 4.6 & 1 & 5.2 & 15 & 1.2 & 0 & 5.5 & 0 & 3.8 & 0 & 4.2 & 0 & 2.0 & \textbf{1} & 3.6 & 24 & 4.0 & \textbf{40} & 11. & 35 & 5.8 & 17 & 9.1\\
AdHesAf & \textbf{33} & 5.7 & 2 & 7.6 & 35 & 2.9 & 0 & 7.2 & \textbf{1} & 6.5 & 0 & 6.0 & 0 & 3.2 & \textbf{1} & 4.9 &25 & 5.4 & \textbf{40} & 10. & 35 & 7.2 & 18 & 13.\\
\hline
\multicolumn{25}{|c|}{Affine adaptation}\\
\hline
DoG & 29 & 2.3 & 0 & 2.8 & 10 & 0.8 & 0 & 2.7 & 0 & 2.3 & 0 & 2.1 & 0 & 1.0 & \textbf{1} & 2.4 & 13 & 2.0 & 38 & 4.8 & 29 & 2.7 & 12 & 4.7\\
DoGAf & 26 & 2.3 & 0 & 2.5 & 9 & 0.8 & 0 & 2.7 & 0 & 2.2 & 0 & 2.1 & 0 & 1.0 & \textbf{1} & 1.8 & 6 & 2.0 & 39 & 3.8 & 22 & 2.7 & 12 & 4.8\\
%Hes & \textbf{33} & 3.6 & 1 & 6.3 & 26 & 1.6 & \textbf{2} & 5.9 & \textbf{1} & 4.2 & 0 & 4.4 & 0 & 2.2 & 1 & 3.5 & - & - & 39 & 8.6 & \textbf{37} & 6.8 & \textbf{18} & 9.9\\
%HesAf & 32 & 4.6 & 1 & 5.2 & 15 & 1.2 & 0 & 5.5 & 0 & 3.8 & 0 & 4.2 & 0 & 2.0 & \textbf{1} & 3.6 & 24 & 4.0 & \textbf{40} & 11. & 35 & 5.8 & 17 & 9.1\\
SURF & 27 & 2.3 & 0 & 2.4 & 7 & 1.0 & 0 & 2.5 & 0 & 1.9 & 0 & 2.1 & 0 & 0.9 & \textbf{1} & 1.4 & 10 & 1.9 & 38 & 5.8 & 31 & 2.9 & 15 & 4.0\\
SURFAf & 22 & 2.2 & 1 & 2.0 & 7 & 0.9 & 0 & 2.6 & 0 & 1.6 & 0 & 1.7 & 0 & 0.8 & \textbf{1} & 1.3 & 6 & 1.7 & \textbf{40} & 6.2 & 21 & 2.4 & 12 & 4.0\\
KAZE & 28 & 4.3 & 0 & 3.6 & 10 & 0.8 & 1 & 4.7 & 0 & 3.4 & 0 & 4.0 & 0 & 1.3 & \textbf{1} & 2.7 & 25 & 3.6 & 38 & 13. & 35 & 5.6 & 17 & 6.4\\
KAZEAf & 28 & 2.5 & 1 & 3.4 & 7 & 0.8 & 0 & 4.8 & \textbf{1} & 3.3 & 0 & 3.8 & 0 & 1.4 & \textbf{1} & 2.8 & 21 & 3.5& 39 & 6.1 & 33 & 5.7 & 15 & 8.2\\
FOCI & 29 & 12. & 0 & 39. & 14 & 11. & 1 & 32. & 0 & 29. & 0 & 29. & 0 & 20. & \textbf{1} & 29. &21 & 13.& 38 & 35. & 35 & 27. & 17 & 45.\\
FOCIAf & 21 & 11. & 1 & 17. & 3 & 5.8 & 0 & 15. & 0 & 11. & 0 & 13. & 0 & 10. & 0 & 6.0 &  7 & 12.& 37 & 19. & 19 & 14. & 12 & 27.\\
\hline
\multicolumn{25}{|c|}{Other detectors}\\
\hline
ORB & 3 & 4.1 & 0 & 3.6 & 1 & 0.8 & 0 & 2.8 & 0 & 2.7 & 0 & 3.6 & 0 & 1.6 & 0 & 2.8 & 1 & 2.3 & 28 & 8.7 & 5 & 3.0 & 3 & 6.1\\
SFOP & 26 & 9.3 & 0 & 16. & 12 & 4.7 & 0 & 12. & 0 & 10. & 0 & 10. & 0 & 9.2 & 0 & 7.5 & 11 & 12. & 36 & 15. & 24 & 11. & 8 & 17.\\
WADE & 16 & 14. & 0 & 20. & 0 & 3.4 & 0 & 58. & 0 & 11. & 0 & 14. & 0 & 7.9 & \textbf{1} & 8.3 & 20 & 23. & 34 & 60. & 34 & 46. & 13 & 77.\\
W$\alpha$SH & 0 & 1.8 & 0 & 5.4 & 0 & 0.6 & 0 & 2.8 & 0 & 2.5 & 0 & 1.4 & 0 & 1.8 & 0 & 1.2 & 0 & 1.9 & 24 & 4.1 & 3 & 2.8 & 3 & 6.9\\

